Interaction Embeddings for Prediction and Explanation in Knowledge Graphs

Knowledge graph embedding aims to learn distributed representations for entities and relations, and is proven to be effective in many applications. Crossover interactions --- bi-directional effects between entities and relations --- help select related information when predicting a new triple, but haven't been formally discussed before. In this paper, we propose CrossE, a novel knowledge graph embedding which explicitly simulates crossover interactions. It not only learns one general embedding for each entity and relation as most previous methods do, but also generates multiple triple specific embeddings for both of them, named interaction embeddings. We evaluate embeddings on typical link prediction tasks and find that CrossE achieves state-of-the-art results on complex and more challenging datasets. Furthermore, we evaluate embeddings from a new perspective --- giving explanations for predicted triples, which is important for real applications. In this work, an explanation for a triple is regarded as a reliable closed-path between the head and the tail entity. Compared to other baselines, we show experimentally that CrossE, benefiting from interaction embeddings, is more capable of generating reliable explanations to support its predictions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-sigconf-authordraft.tex \
	samples/sample-sigconf-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-sigconf-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done

samples/sample-manuscript.pdf \
samples/sample-acmsmall.pdf \
samples/sample-acmlarge.pdf \
samples/sample-acmtog.pdf: samples/samplebody-journals.tex

samples/sample-sigconf.pdf \
samples/sample-sigconf-authordraft.pdf \
samples/sample-sigconf-xelatex.pdf \
samples/sample-sigplan.pdf \
samples/sample-sigchi.pdf: samples/samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean
	$(RM) $(PDF) samples/*-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.


==> T-DSE-compare.tex <==
\begin{table}[!htb]
\centering
\footnotesize
\caption{}
\label{DSE compare }
  \begin{tabular}{| p{1.7cm} |p{1.2cm} | p{1.2cm}| p{1.2cm} | p{1.2cm}| }
    \hline

       \multicolumn{1}{|c|}{Method}  &\multicolumn{1}{|c|}{MR} & \multicolumn{1}{|c|}{H10(\%)}  & \multicolumn{1}{|c|}{H3(\%)} & \multicolumn{1}{|c|}{H1(\%)} \\
      %\cline{2-5} &\multicolumn{1}{|c|}{Raw}   &\multicolumn{1}{|c|}{Filter}  &\multicolumn{1}{|c|}{Raw}   &\multicolumn{1}{|c|}{Filter} \\
     %\cline{2-9}& \multicolumn{1}{|c|}{Raw} & \multicolumn{1}{|c|}{Filter} & \multicolumn{1}{|c|}{Raw} & \multicolumn{1}{|c|}{Filter} & \multicolumn{1}{|c|}{Raw} & \multicolumn{1}{|c|}{Filter} & \multicolumn{1}{|c|}{Raw} & \multicolumn{1}{|c|}{Filter} \\
    \hline
    basic               &      340/185     &     52.2/74.0     &    29.0/63.6      &     10.4/21.2     \\
    +linear             &      297/138     &     49.8/75.4     &    27.8/63.8      &     13.9/43.3     \\
    +bilinear           &                  &                   &                   &                   \\
    +nonlinear          &                  &                   &                   &                   \\
    +dropout(DSE)       &      194/41      &     53.0/84.2     &    30.9/70.6      &     15.6/48.4     \\

    % python3 DSE.py --max_iter 100 --eval_per 10 --neg_weight 50 --batch 4000 --lr 0.01 --dim 200 --loss_weight 1e-4 ./output/0112result4.file
    
    \hline

  \end{tabular}
  \end{table}

==> T-diverse-semantic.tex <==
\begin{table*}[!htb]
\centering
\footnotesize


  \begin{tabular}{| c |c | c | l | }
  \hline
  Semantic & Dataset summary & OWL2 axiom  & axiom condition\\
  \hline
  Class & \s{$x\%$ classes/entity}
  & \s{$\texttt{ClassAssertion(C a)}$} 
  & \s{$(\texttt{a})^\texttt{I} \in (\texttt{CE})^\texttt{C}$} \\
  % & \s{e(/m064jjy):C(/tv/tv\_director), C(/film/actor), C(/tv/tv\_wrtiter)}  
  %\hline
  Domain &\s{ $52.6\%$ relations has explicit domain}  
  & \s{\texttt{ObjectPropertyDomain(OPE$_\texttt{1}$ OPE$_\texttt{2}$)}} 
  & \s{$\forall \texttt{x},\texttt{y}:(\texttt{x},\texttt{y})\in(\texttt{OPE})^{\texttt{OP}}   \Rightarrow  \texttt{x} \in (\texttt{CE})^\texttt{C}$}  \\
  % \s{$ObjectPropertyDomain(\texttt{OPE} \; \texttt{CE})$}
  %& \s{\texttt{$\forall$ x,y:(x,y)$\in$(OPE)$^{\texttt{OP}}$   $\Rightarrow$  x $\in$ (CE)$^\texttt{C}$}}
  % & \s{r(/theater\_roles.): domain(/theater/theater\_role/role)}
  %\hline
  Range & \s{$52.6\%$ relations has explicit range} 
  &\s{\texttt{ObjectPropertyRange(OPE CE)}} 
  & \s{$\forall \texttt{x},\texttt{y}:(\texttt{x},\texttt{y})\in(\texttt{OPE})^{\texttt{OP}}   \Rightarrow  \texttt{y} \in (\texttt{CE})^\texttt{C}$} \\
  % & \s{r(/theater\_roles.): range(/theater/theater\_actor)}
  %\hline
  Inverse & \s{$100\%$ relations has inverse relations in theory } 
  & \s{\texttt{InverseObjectProperties(OPE$_\texttt{1}$ OPE$_\texttt{2}$)}}  
  & \s{$(\texttt{OPE})_\texttt{1}^{\texttt{OP}} = \{ (\texttt{x,y})| \texttt{(y,x)} \in (\texttt{OPE}_\texttt{2}^{\texttt{OP}}) \}$ } \\
  %&\s{r(/people/person/parents): inverse(/people/person/chlidren)}
  %\hline
  Reflexive & \s{$x\% $ C1 structures}   
  &\s{\texttt{RefxiveObjectProperty(OPE)}} 
  &  \s{$\forall \texttt{x:x} \in \Delta _{\texttt{I}} \Rightarrow (\texttt{x,x}) \in (\texttt{OPE}^{\texttt{OP}} ) $ } \\
  %\hline
  Symmetric & \s{$x\%$ C2 structures}  
  &\s{\texttt{SymmetricObjectProperty(OPE)}} 
  & \s{$\forall \texttt{x,y} \in (\texttt{OPE}^{\texttt{OP}})  \Rightarrow (\texttt{y,x}) \in (\texttt{OPE}) ^{\texttt{OP}}$ } \\
  %\hline
  \multirow{2}{*}{Transitive} & \multirow{2}{*}{\s{$x\%$ C3 structures} } 
  &\multirow{2}{*}{\s{\texttt{TransitiveObjectProperty(OPE)}} }
  &  \s{$ \forall \texttt{x,y,z} : (\texttt{x,y}) \in (\texttt{OPE}) ^{\texttt{OP}} \texttt{and} (\texttt{y,z}) \in (\texttt{OPE}) ^{\texttt{OP}} $ } \\
  &  &    &\s{ $ \; \; \; \; \; \; \; \; \; \; \; \; \; \;  \Rightarrow (\texttt{x,z}) \in (\texttt{OPE}) ^{\texttt{OP}}$} \\
  %\hline
  \multirow{3}{*}{Cardinality} & \s{$26.2\%$ 1-1 relations}  
  &\s{\texttt{ObjectMinCardinality(n OPE)}} 
  & \s{ $\{ \texttt{x} | \# \{\texttt{y}| (\texttt{x,y}) \in (\texttt{OPE}) ^{\texttt{OP}} \texttt{and} \texttt{y} \in (\texttt{CE}) ^{\texttt{C}} \ge \texttt{n}   \} $}  \\
  		
  & \s{$22.7\% \; 28.3\%$ 1-N, N-1 relations} 
  &\s{\texttt{ObjectMaxCardinality(n OPE)}} 
  & \s{ $\{ \texttt{x} | \# \{\texttt{y}| (\texttt{x,y}) \in (\texttt{OPE}) ^{\texttt{OP}} \texttt{and} \texttt{y} \in (\texttt{CE}) ^{\texttt{C}} \le \texttt{n}   \} $}   \\


  & \s{ $22.8\%$ N-N relations} 
  &\s{\texttt{ObjectExactCardinality(n OPE)}} 
  & \s{ $\{ \texttt{x} | \# \{\texttt{y}| (\texttt{x,y}) \in (\texttt{OPE}) ^{\texttt{OP}} \texttt{and} \texttt{y} \in (\texttt{CE}) ^{\texttt{C}} = \texttt{n}   \} $}  \\
\hline

  \end{tabular}

 	\caption{Diversity of semantic in knowledge base}
	\label{diverse semantic}
  \end{table*}

==> T-domain-range.tex <==
\begin{table*}[!htb]
\footnotesize
\centering
\begin{tabular}{|c |l| l|}
\hline
relations  & Top 3 nearest relations  & Top 3 nearest relations for inverse relation\\
\hline
\multirow{3}{*}{/people/person/children} & /people/person/parents & /people/person/parents\\
 \cline{2-3}  & /people/person/.../sibling\_relationship/sibling   & /people/person/spouse\_s./.../marriage/spouse\\ 
  \cline{2-3} & /people/person/spouse\_s./.../marriage/spouse   & /people/person/.../sibling\_relationship/sibling \\ 
  %\cline{2-3} & /celebrities/.../celebrities/friendship/friend     & /celebrities/.../romantic\_relationship/celebrity\\
  %\cline{2-3} & /influence/influence\_node/influencedd             & /celebrities/.../romantic\_relationship/celebrity\\ 
\hline
\multirow{3}{*}{/tv/tv\_program/languages} & /film/film/language   & /tv/tv\_program/genre \\
 \cline{2-3}  & /film/actor/.../dubbing\_performance/language      & /tv/tv\_program/original\_network./.../network  \\ 
  \cline{2-3} & /people/person/languages                           & /tv/tv\_program/country\_of\_origin \\ 
  %\cline{2-3} & /base/schemastaging/.../service\_language          & /tv/tv\_program/spun\_off\_from\\
  %\cline{2-3} & /people/ethnicity/languages\_spoken                & /tv/tv\_program/.../regular\_tv\_appearance/character\\
\hline

\multirow{3}{*}{/sports/sports\_team/location} & /music/artist/origin &  /sports/sports\_team\_location/teams\\
 \cline{2-3}  & /people/deceased\_person/place\_of\_death          & /organization/organization/place\_founded\\ 
 \cline{2-3}  & /organization/.../mailing\_address/citytown        & /education/educational\_institution/.../student \\
  %\cline{2-3} & /people/person/place\_of\_birth                    & /sports/professional\_sports\_team/.../school \\ 
  %\cline{2-3} & /location/.../adjoining\_relationship/adjoins      & /business/employer/.../employment\_tenure/person \\
\hline
 \end{tabular}
\caption{Top 3 nearest relations }
 \label{relation type result}
\end{table*}



==> T-inference-chain.tex <==
\begin{table*}[!htp]
\centering
\footnotesize
\begin{tabular}{|l| l|l|l|}
\hline
\multicolumn{3}{|c|}{for relation XXX} \\
\hline
seed entity & similar entities & inference chain for (a, r1, b) & inference chain for entity \\
\hline
entity 1  & entity1, entity3, entity4 & (a, r1, b) $\land$  (a, r1, b) $\Rightarrow$ (a, r1, b) & triple1, triple2, triple3 \\
\hline 
entity 1  & entity1, entity3, entity4 & (a, r1, b) $\land$  (a, r1, b) $\Rightarrow$ (a, r1, b) & triple1, triple2, triple3\\
\hline 
entity 1  & entity1, entity3, entity4 & (a, r1, b) $\land$  (a, r1, b) $\Rightarrow$ (a, r1, b) & triple1, triple2, triple3\\

\hline


\end{tabular}
\label{inference chain}

\end{table*}

==> T-similar-entities.tex <==
\begin{table}[!htp]
\centering
\begin{tabular}{|l| l|}
\hline
\multicolumn{2}{|c|}{for entity Toronto} \\
\hline
with relation  & similar entities \\
\hline
\multirow{3}{*}{/location/location/time\_zones} & Montreal  \\
					&Berlin	\\
					&Reading	\\
\hline
\multirow{3}{*}{/capital\_of.} & Hamilton  \\
					&Ottawa	\\
					&London	\\
\hline
\multirow{3}{*}{/location/location/events} & Berlin  \\
					&Sydney	\\
					&Vienna	\\

\hline


\end{tabular}
\label{similarEntity}

\end{table}


\begin{comment}
entid: Toronto 	rel: /location/location/time_zones 	ent_list: ['Toronto', 'Montreal', 'Berlin', 'Reading']  
entid: Toronto 	rel: /location/location/people_born_here 	ent_list: ['Toronto', 'Hamilton', 'Montreal', 'Geneva']  
entid: Toronto 	rel: /location/capital_of_administrative_division/capital_of./location/administrative_division_capital_relationship/administrative_division 	ent_list: ['Toronto', 'Hamilton', 'Ottawa', 'London']  
entid: Toronto 	rel: /base/biblioness/bibs_location/country 	ent_list: ['Toronto', 'Montreal', 'Potsdam', 'Turin']  
entid: Toronto 	rel: /travel/travel_destination/how_to_get_here./travel/transportation/transport_operator 	ent_list: ['Toronto', 'Oslo', 'Berkeley', 'Ottawa']  
entid: Toronto 	rel: /location/location/contains 	ent_list: ['Toronto', 'Hamilton', 'London', 'Montreal']  
entid: Toronto 	rel: /location/location/adjoin_s./location/adjoining_relationship/adjoins 	ent_list: ['Toronto', 'Virginia', 'Ontario', 'Manitoba']  
entid: Toronto 	rel: /film/film_location/featured_in_films 	ent_list: ['Toronto', 'Geneva', 'Sydney', 'Montreal']  
entid: Toronto 	rel: /common/topic/webpage./common/webpage/category 	ent_list: ['Toronto', 'Ottawa', 'Geneva', 'Vancouver']  
entid: Toronto 	rel: /base/popstra/location/vacationers./base/popstra/vacation_choice/vacationer 	ent_list: ['Toronto', 'Ottawa', 'Italy', 'Frankfurt']  
entid: Toronto 	rel: /sports/sports_team_location/teams 	ent_list: ['Toronto', 'Montreal', 'Sydney', 'Hilversum']  
entid: Toronto 	rel: /base/biblioness/bibs_location/state 	ent_list: ['Toronto', 'Montreal', 'Ottawa', 'Savannah']  
entid: Toronto 	rel: /travel/travel_destination/climate./travel/travel_destination_monthly_climate/month 	ent_list: ['Toronto', 'Sydney', 'Ottawa', 'Geneva']  
entid: Toronto 	rel: /location/administrative_division/second_level_division_of 	ent_list: ['Toronto', 'Osaka', 'London', 'Vietnamese_Language']  
entid: Toronto 	rel: /travel/travel_destination/how_to_get_here./travel/transportation/mode_of_transportation 	ent_list: ['Toronto', 'Ottawa', 'Victoria', 'Hilversum']  
entid: Toronto 	rel: /location/location/events 	ent_list: ['Toronto', 'Berlin', 'Sydney', 'Vienna']  
entid: Toronto 	rel: /location/location/containedby 	ent_list: ['Toronto', 'Hamilton', 'London', 'Ottawa']
\end{comment}

==> T-triple-classification.tex <==
\begin{table}[!htb]
\centering
\caption{Triple classification result}
 \label{triple classification result}
\begin{tabular}{|c |c| c|}
\hline
Data set & WN11 & FB13 \\
SE  & 53.0 & 75.2 \\
TransE\_u & 75.9 & 70.9 \\
TransE\_b & 75.9 & 81.5 \\
TransH\_u & 77.7 & 76.8 \\
TransH\_b & 78.8 & 83.3 \\
\textbf{DSE} &   &   \\
TransR\_u & 85.5 & 74.7 \\
TransR\_b & 85.9 & 82.5 \\

\hline
 \end{tabular}
\end{table}

==> T-type-percent.tex <==
\begin{table*}[!htbp]
\centering
  \begin{tabular}{ c| c| c| c| c| c|c| c| c| c| c| c| c}
  \toprule
   & \multicolumn{2}{|c|}{type 1}  & \multicolumn{2}{|c|}{type 2}  & \multicolumn{2}{|c|}{type 3}& \multicolumn{2}{|c|}{type 4}  & \multicolumn{2}{|c|}{type 5}  & \multicolumn{2}{|c}{type 6}\\
   \cline{2-13}
   & \emph{AvgS.} & \emph{Percent} & \emph{AvgS.} & \emph{Percent} & \emph{AvgS.} & \emph{Percent} & \emph{AvgS.} & \emph{Percent} & \emph{AvgS.} & \emph{Percent} & \emph{AvgS.} & \emph{Percent} \\
   \hline
TransE &  8.38 & 0.14 & 0.00 & 0.00  & 0.01 & 0.00 & 0.01 & 0.00 &\textbf{26.94} &  \textbf{0.44}&25.99  & 0.42\\
\hline
ANALOGY &  \textbf{2.57} & \textbf{0.51} & 2.16 & 0.43  & 0.13 & 0.03 & 0.14 & 0.03 &0.01 & 0.00 &0.01  & 0.00\\
\hline
CrossE &  6.38 & 0.01 & 4.31 & 0.01  & 55.07 & 0.10 & 54.89 & 0.10 &\textbf{222.83} & \textbf{0.39} &222.76  &0.39 \\
\bottomrule

\end{tabular}
\caption{The \emph{AvgSupport} and percent of explanations belonging to each type of similar structure. The numbers marked in bold correspond to the highest \emph{AvgSupport} and percent of each KGE.}
\label{type-percent}
\vspace{-3mm}
\end{table*}



\begin{table}
	\centering
	\begin{tabular}{c| c| c|c| c| c|c }
	\toprule
	 & \multicolumn{3}{|c|}{first top type} & \multicolumn{3}{|c}{second top type}\\
	 \hline
	 		& type  & AvgS. & Perc.  & type  & AvgS. & Perc. \\
	 \hline
	 TransE & type 5 & 26.94 & 0.44 & type 6 &25.99 & 0.42 \\
	 \hline
	 ANALOGY & type 1 & 2.57 & 0.51 & type 2 &2.16 & 0.43 \\
	 \hline
	 CrossE & type 5 & 222.83 & 0.39 & type 6 &222.76 & 0.39 \\
		
	\end{tabular}
\end{table}


==> case-stardy-with-similarity.tex <==
\subsection{Case Study of Crossover Information Selection with/in CrossE}
We have shown CrossE is more capable of modeling individual triples via link prediction experiment and is capable of capturing high-level semantic in knowledge graph using inverse/symmetric/reflexive as examples. In this section, we present some examples of \emph{crossover embeddings}  to show CrossE really simulate the \emph{crossover information selection} between entities and relations.

\subsubsection{Entity Infomation Selection}
To evaluate the entity information selection results, we compare different crossover embeddings of entities. 
For each entity $e$, it has $n_r$ crossover embeddings, in which $n_r$ is the number of relations in knowledge graph. 
Each entity corssover embedding is a representation of the entity selected information with one relation.

\emph{ For one entity, it's crossover embeddings with relations of same domain should be similar.} 
Because with one relation, the related information to selected for an entity is highly related with the domain of relation, 
as showed in \wen{......}. 
To illustrate this, we take two entities from FB15k, \emph{The Germain Empire} and \emph{Peter Berg}, and get their crossover embeddings with different relations. We use T-SNE~\cite{TSNE:journal/JMLR/2008} to do dimensionality reduction and visualize them in Figure \ref{projected entity}. We only visualize the crossover embeddings with relations that the entity is linked with. Figure \ref{projected entity} shows that for one entity 
(1) the crossover embeddings are various with regard to different relations. This proves that the information of an entity is various and information selection is necessary.
(2) the crossover embeddings are more similar if they correspond to relations with same domain topic. This shows that CrossE succefully simulate the entity information selection with regard to different relation.

\begin{figure}[!htbp] 
\centering 
%/m/03b79
\subfigure[The German Empire]{
	\label{entityProducted1}
	\includegraphics[scale=0.25]{Figure_21.png}
}
\subfigure[Peter Berg]{
	\label{entityProducted2}
	\includegraphics[scale=0.25]{Figure_11.png}
}

\caption{ Visualization for interaction embeddings of two entity. Each cross is an interaction embedding with one relation. Different colors represent various topic of relation domain. The topic of relation domain is generated by selecting the first word in relation string. }
\label{projected entity} 
%\vspace{-3mm}
\end{figure} 

\begin{comment}
\emph{With regard to different relations, the most similar crossover embeddings of other entities with an entity's crossover embedding should be different.} Because the similarity of two crossover embeddings is correspond to the similarity of two enities based on selected information. Thus the similarity of two entities will vary with different relations. To illustrate this, we take one entity and select the top $3$ similar entities via their crossover embeddings with two different relations. The results are shown in Table \ref{similarEntity}. The similar entity list are different shows that 
(1) different relation focus on different information of one entity.
(2) CrossE succefully simulate the entity information selection.
\input{T-similar-entities}
\end{comment}

\input{T-inference-chain}

\subsubsection{Relation Information Selection}
To evaluate the relation information selection, we compare different crossover embeddings of relations. For each relation $r$, there are $n_e$ crossover embeddings. $n_e$ is the number of entities in knowledge graph.
Each relation crossover embedding is a representation of the relation selected information with one entity.
We regard the selected information of relations as the inference chains, which is a path from head entity to tail entity.

\emph{The inference chain of one relation is different based on the selected information of entity, thus for entities whose selected information are similar, their inference chain with the relation are more likely to be same.} For one relation, we calculate all possible crossover embeddings for it based on the (head enitty, relation) pair exists in training data. Then we an entity and calculate its top $k$ similar entities based on the their relation crossover embeddings. We regard these $k+1$ entities are with the same inference chain. And we regard inference chain as the most common path among these entitise in knowledge graph to infer  the relation.


==> high-level-semantics.tex <==
\subsection{High-level Semantic Capturing}
As CrossE using crossover embeddings as the representation for entities and relations while involving specific triples.
It is more easier for general embeddings to capture high-level semantics. 
In this section, we evaluate the CrossE on high-level semantic capturing, using inverse relations, reflexive and symmetric relations as examples.
%A good embedding model should capture the semantics  existing in a knowledge graph.
In this section, we show that with CrossE, we move a step towards semantic discovery.
The evaluation are based on the embedding results of denser dataset, FB15k.
%These evaluation are on the denser of two datasets, FB15k.
\begin{comment}
\subsubsection{1-1, 1-N, N-1, and N-N Relations}
%\CHJ{just comment: for the experiment analysis for 1-N, N-N relation, could we rephrase it from the perspective of cross-over interaction.}
We evaluate the link prediction H10 results on FB15k with \emph{Filter} setting via mapping the relation into 1-1, 1-N, N-1 and N-N following the same metric as previous methods. 
% There are $26.2\%$ 1-1 relations, $22.7\%$ 1-N relations, $28.3\%$ 1-N relations and $22.8\%$ N-N relations. 
The results are listed in Table~\ref{relation type result}.
%We evaluate the capability of CrossE to encode the cardinality semantic, Table \ref{relation type result} show the separate H10 results on FB15k by mapping relations into 1-1, 1-N, N-1 and N-N classes following the same matric in  TransE\cite{}. There are $26.2\%$ 1-1 relations, $22.7\%$ 1-N relations, $28.3\%$ 1-N relations and $22.8\%$ N-N relations.
%The results are the average H10 rate of head prediction and tail prediction. 
\input{T-relation-type-result}
%
%\input{T-domain-range}
Table \ref{relation type result} shows that CrossE significantly outperforms other embedding methods and CrossE$_S$ in 1-N, N-1, and N-N relations which are the three most common and important types 
%because there are $1.4\%$ triplets are related with 1-1 relations, $8.9\%$ related with 1-N relations, $14.6\%$ related with N-1 relations and $75.1\%$ related with N-N relations.
% from the perspective of number of triples related with these types. 
because there are $1.4\%$, $8.9\%$,$14.6\%$ and $75.1\%$ triples related with 1-1, 1-N, N-1, and N-N relations respectively in the test dataset.
It means that majority of triples are related with N-N relations and the prediction results on N-N relations will influence the final results the most. 
\end{comment}


%are related with 1-1 relations, $8.9\%$ related with 1-N relations, $14.6\%$ related with N-1 relations and $75.1\%$ related with N-N relations. So the majority of triples are related with N-N relations and the prediction results on N-N relations will effect the final results most.
%\input{T-DSE-compare}
%\subsection{Triplet classification}
%\input{T-triple-classification}

%\subsection{Semantic Discovery}

%\CHJ{I feel Semantic Discovery is not a good phrase, are there any other candidate?}\wen{Detection?}
%A good embedding model should be capable of capturing the semantics  existing in knowledge graph data.
%In this section, we show that with CrossE, we move a step to semantic discovery.
%These semantic discovery experiments are on the denser of two datasets, FB15k 

% as it has more relations and is more dense than WN18.
%In this section, we evaluate DSE on whether it is capable to encode the diverse semantic analysed in Section 3 on FB15k as it has more relaitons and is more dense than WN18. 

\begin{comment}
\begin{figure*}[htbp] 
\centering 
%/m/03b79
\subfigure[The German Empire]{
	\label{entityProducted1}
	\includegraphics[scale=0.24]{Figure_21.png}
}
\subfigure[Peter Berg]{
	\label{entityProducted2}
	\includegraphics[scale=0.24]{Figure_11.png}
}
\subfigure[/../medals\_won./...]{
	\label{relationProducted1}
	\includegraphics[scale=0.24]{relation_1.png}
}
\subfigure[/broadcast/artist/content]{
	\label{relationProducted2}
	\includegraphics[scale=0.24]{relation_3.png}
}
\caption{ \ref{entityProducted1} and \ref{entityProducted2} are two visualization examples for entities' interaction embeddings. Each cross is an interaction embedding with one relation. Different colors represent various topic of relation domain. The topic of relation domain is generated by selecting the first word in relation string. \ref{relationProducted1} and \ref{relationProducted2} are two examples for the correlation between the information overlap and the similarity of relation crossover interaction embeddings for one entity pair. Each dot is an entity pair.}
\label{projected entity} 
%\vspace{-3mm}
\end{figure*} 
\end{comment}

\begin{comment}
\subsubsection{Domain and Range of Relations }
Domain and range are two basic semantics for relation in knowledge graph which specify the classes of head and tail respectively for a given relation.
%\input{T-domain-range}
We first generate the domain and range for every relation. 
%\CHJ{Domain and range specify the types of head and tail respectively for a given relation.}
In Freebase, a relation string contains many words connected  with '/' and could be classified into two types:
strings with a word ended with a dot in the middle like \emph{/common/topic/webpage./common/webpage/topic} and strings without dot like $/film/film/music$. The string with a dot in the middle is always a predicate and we call it \emph{predicate word}. 
%We generate domain/range for these two types of strings following different rule:
For the relation string with predicate word, we regard the word before predicate word as domain and the last word as range.
%for the strings with dot, we choose the word before \emph{dot word} as domain string and the last word of the whole string as range;
For the strings without predicate word, we choose the first word as domain and the last word as range.
As there are many selected domain/range texts connected with `\_', such as \emph{appointed\_by} and they are not a subclass name, 
so we replace these domain and range strings as `NULL' and call this as  \emph{Filter} setting, and the original as \emph{Raw} setting.
After filtering, there are $554$ relations whose domain is `NULL' and $581$ relations whose range is `NULL'.
%If the selected domain/range strings many words connected with '\_', such as \emph{basic\_title}, we choose the last word as result.
%After generating the domain/range automatically, we also check the results  and correct some wrong results manually as there also exists strings like \emph{directed\_by}. 

The assumption is that the relations with same domain and range are similar and should be close in the embedding space. To evaluate the capability of encoding the semantics of domain and range, for each relation $r$ we select the top $2$ and $5$ most similar relations and check the overlap of their domains and ranges. 
As CrossE has one general embedding and one inverse embedding for a relation, we select the most similar entities through their general embedding when computing the range overlap and select the most similar entities through their inverse embedding when computing the domain overlap. 
The final result is the average overlap of domain/range for all relations and listed in Table \ref{domain/range results}.


\begin{table}[!htb] 
\footnotesize
\centering
 \begin{tabular}{ |p{0.9cm} |p{1.35cm} p{1.35cm} | p{1.35cm} p{1.35cm} |}
\hline
\multirow{2}{*}{Method}  & \multicolumn{2}{|c|}{Domain overlap (\%)} & \multicolumn{2}{|c|}{Range  overlap (\%)} \\
\cline{2-5} 	& \multicolumn{1}{|c|}{Top2} 	&\multicolumn{1}{|c|}{Top5}   	& \multicolumn{1}{|c|}{Top2}  & \multicolumn{1}{|c|}{Top5} 		\\
\hline
TransE  		& 	60.3 / 78.3	& 33.4 / 50.5		& 	58.4 / 78.5	&	32.1 / 52.9		\\

\textbf{CrossE} 	&  \textbf{70.2} / 83.0		& \textbf{46.4} / \textbf{62.3}	& 	\textbf{62.4} / 82.4	& \textbf{35.3} / 56.9	\\
\textbf{CrossE$_S$}&	65.1 / \textbf{85.5}			&	36.2 / 56.3			&	61.9 / \textbf{86.0}		&		34.7 / \textbf{62.8}		\\
\hline
\end{tabular}
\caption{Evaluation results for domain/range overlap. The results on the the left of "/" is with \emph{Raw} setting and the right with \emph{Filter}.}
\label{domain/range results}
\vspace{-3mm}
\end{table}
\end{comment}

%From Table \ref{domain/range results}, we could conclude that 1) CrossE$_S$ significantly outperforms TransE especially with \emph{Filter} setting and this illustrates the efficiency of nonlinear and multiple negative sampling as they are the major difference between TrasnE and CrossE$_S$; and 2) CrossE outperforms Cross$_S$ in all \emph{Raw} settings and one \emph{Filter} setting which illustrate the efficiency of CrossE to catch complex semantic of relations.

\subsubsection{Inverse Relations}\wen{shall we remove this part? it's too confusing}
Inverse is a common semantic for relations. 
For example, \emph{isChildOf} is the inverse relation of \emph{isFatherOf}.

To find inverse relation pairs, we based on the assumption that 
the general inverse embedding of one relation should be close to the general embedding for its inverse relation.
%inverse relation pairs should be close to each other in the embedding space.
%To evaluate the capability of CrossE to encode the inverse relation semantic.
%We generate inverse relation pairs according to general relation embedding and then check the correctness manually as there are no labeled inverse relation pairs.
For each relation, we generate the inverse relation by selecting the most similar relation through cosine similarity between other relation's general embedding and the inverse embedding of current relation. 
We select right pairs utilizing the symmetric property of inverse relation pair which means if $r_1$ is the inverse relation of $r_2$, then $r_2$ is the inverse relation of $r_1$. \wen{the assumption is wrong, inverse relation is not symmtric. Think \emph{isChildOf} and \emph{isFatherOf}}
If the inverse relation of  $r_x$ is $r_y$, $r_y$ is a different with $r_x$, and the inverse relation of $r_y$ is $r_x$, then we regard the inverse pair ($r_x, r_y$) is correct. We check the correctness manually as there are no labeled inverse relation pairs. Finally, we get $409$ inverse relation pairs which covers $60.8\%$ relations in FB15k and the correctness is $93.2\%$.
Table \ref{inverse relation} shows the similarity scores of some examples of inverse relation pairs.
\input{T-inverse-relation}


\subsubsection{Reflexive and Symmetric Relations}
CrossE is capable of discovering the reflexive and symmetric relations which are another two important semantics for relations. If one relation $r$ is reflexive, then there exists $( e, r, e )$. The inverse triple for  $( e, r, e )$ is $( e, r^{-1}, e )$ and we could conclude that the embedding of a reflexive relation $r$ and the inverse embedding of $r$ in CrossE must be similar. The same conclusion also could be inferred  for symmetric relations. 

For each relation, we get the possible inverse relation pair as before and 
select all relations that the most similar inverse relation is itself. 
Finally, we get $103$ relations.
To evaluate the correctness of the selected relations,
we retrieve the related triples in training data for each $r$ in the selected relations. If more than $50\%$ head tail entity pairs that $(h,r,t)$ and $(t,r,h)$ both exist, we regard $r$ as a exactly true symmetric relation. If there are more than $50\%$ triples of the relation $r$ which the head entity is the same with tail entity, we regard $r$ as exactly true reflexive relation.
Among those $103$ relations, there are $51$ exactly true symmetric relation and $10$ exactly true reflexive relation which means the correctiveness is $59.2\% +$. 
Table \ref{symmetric relation} are five examples of these relations.
\input{T-symmetric}


==> motivationAnalysis.tex <==
%!TEX root = crosse_cikm18.tex
\section{Crossover Interactions and Inference with C\lowercase{ross}E}%\wen{should we remove this part? there are examples in introduction and the explanation with OWL is quite confusing}
\label{sec:crossover}
Before introducing our KGE CrossE in subsequent sections, we explain crossover interactions and the rationale for considering them in this section.

During inference, the crossover interactions between entities and relations help select relevant information. Such interactions go both way: from relations to entities, and from entities to relations.
The relation participating in a triple determines the relevant information to be selected about the participating entities, which we refer as \emph{entity selection}.
On the other hand, the participating entities also determine the relevant relations to be selected, which we refer as \emph{relation selection.}
In this work we aim to model these bidirectional dependencies and effects between entities and relations, i.e., crossover interactions.

%and explain the concept of  by describing the crossover effects of entities and relations on the triples containing them.
\begin{comment}
To do so, we use axioms in OWL 2~\cite{owl2}, an ontology language for Semantic Web with formally defined meaning, as examples to illustrate the existence of crossover interactions.
\end{comment}

%during inference that only a part of the information for the head entity and relation are involved during tail entity prediction.
%majority existing KGE methods directly learn a general embedding for each entity and relation which \underline{assumed/supposed} to perserve all information of corresponding entity or relation. For all triples contained the same entity or relation, the general emebdding is always used as its representation. 
%They ignore the information selection during inference of a triple. 

\textbf{Crossover Interactions.} We use Figure~\ref{story} as a running example for motivating our study.
In Figure~\ref{story} we can see multiple information (triples) about entity X, but only four of them --- (\emph{X, hasWife, Z}), (\emph{X, fatherIs, Y}), (\emph{Y, isFatherOf, X}), (\emph{S, hasChild, X}) --- are related for the prediction of (\emph{X, isFatherOf, ?}) because they describe family relationships about X and are helpful to infer the father-child relationshiop in (\emph{X, isFatherOf, ?}). The other two triples describe the career of X and will not provide valuable information for this inference task. This is an example of \emph{entity selection} and it depends on the specific relation (e.g., isFatherOf) during inference.

\begin{figure}[htp]
\includegraphics[scale=0.4]{./figures/toyKG2.png}
\caption{A sample knowledge graph. Nodes and edges represent entities and relations. Solid lines represent the triples exist in knowledge graph and dashed lines represent to be predicted triples. }
\label{story}
\end{figure}

In Fig.\ref{story}, there are also multiple information about the relation isFatherOf, e.g., inference chains (\emph{b, fatherIs, a}) $\Rightarrow$ (\emph{a, isFatherOf, b}) and (\emph{a, hasWife, c}) $\land$ (\emph{c, hasChild, b}) $\Rightarrow$ (\emph{a, isFatherOf, b)}. But for the inference of (\emph{X, isFatherOf, ?} ), the inference chain (\emph{a, hasWife, c}) $\land$ (\emph{c, hasChild, b}) $\Rightarrow$ (\emph{a, isFatherOf, b)} is relevant because there is information about \emph{hasWife} for X. This is an example of \emph{relation selection} and it depends on the related information of participating entities during inference. %\wen{should we put this example back to Motivation Analysis?}

Crossover interaction is quite common in knowledge graphs because there are usually various information about every entity and relation. 
%As the information selection of the head entity and relation depend on each other, we name it as \emph{crossove information selection}.
It helps select relevant information and reduce the noise for entity and relation during the inference of a specific triple.
%For example, in Fig \ref{story}, if we want to know ( \emph{X, isFatherOf, ?} ), we first have a look at the information of X and there are 5 triples about X. Among these triples, ( \emph{X, hasWife, Z}), ( \emph{Y, isFatherOf, X}), (\emph{S, hasChild, X}) are related information for us because they both describe the kinship about X, while the other 2 triples describe the career about X and will not provide valuable information for the inference. 

\textbf{Inference Process.} CrossE learns one general embedding for each entity and relation, in addition to an interaction matrix. For inference tasks, the model generates multiple triple specific crossover embeddings using the interaction matrix and general embeddings.
Given an triple $(h, r, t)$, the inference process can be summarized in four steps using the embeddings learned by CrossE: (1) generate \emph{crossover embedding} $\textbf{h}_c$ for head entity $h$, (2) generate \emph{crossover embedding} $\textbf{r}_c$ for relation $r$, (3) combine crossover embeddings $\textbf{h}_c$ and $\textbf{r}_c$, and (4) compare the similarity of combined representation with tail entity embedding $\textbf{t}$. The similarity score computed in the final step is used for determining the feasibility of the triple. %\wen{should we say something about the device of $\textbf{c}_r$?}

The main differences of CrossE compared to existing KGEs are as follows:
% the advantages of CrossE:
(1) For an entity and a relation, the representations used during a specific triple inference are crossover embeddings (not general embeddings), which simulate the selection of different latent properties for different triple predictions.
%and improve the capabiltiy of the general emebdding to capture more deep(global) semantic of it.  
(2) Multiple crossover embeddings for each entity and relation provide richer representations and generalization capability. We argue that they are capable of capturing different latent properties depending on the context of interactions. This is because each crossover embedding can select different similar entities and relations when involving different triples. 
(3) It learns one general embedding for each entity and relation, and uses them to generate crossover embeddings. This results in much less extra parameters than when learning multiple independent embeddings for each entity and relation.

\begin{comment}
KGEs can  perform implicit inferences for knowledge graph completion, while conventional logical reasoning relies upon explicit inference methods.
Viewed this way, the inference capability of embedding method should be an implicit simulation of logic reasoning and capture the underlying semantics and logic. During inference, the crossover interactions between entities and relations help select relevant information. The interactions go both way: from relations to entities, and from entities to relations.

\textbf{Effects to Entities from Relations.}
An entity in a knowledge graph may link to hundreds or thousands of other entities via different relations but only a part of this information is relevant during the inference of a new triple.
For example, the domain and range of a relation specify the classes to which head and tail entities should belong. The corresponding OWL 2 axioms are \emph{ObjectivePropertyDomain()} and \emph{ObjectivePropertyRange()}. Information about domain and range help fetch related information of head entity for a relation.
For example, if we want to do inference on (Steven Spielberg, \emph{directedFilm}, ?), we first search the related information of Steven Spielberg as a director rather than as a father, because the domain of \emph{directedFilm} is \emph{Director}.
Here, the interactions between the relation \emph{directedFilm} and the types of entities affect the information we search during inference. 

\textbf{Effects to Relations from Entities.}
In case of relations, consider their properties like inverse, reflexive, symmetric, and transitive.
These correspond to the OWL 2 axioms \emph{InverseObjectiveProperties()}, \emph{ReflexiveObjectiveProperty()}, \emph{SymmetricObjectiveProperty()} and \emph{TransitiveObjectiveProperty()} respectively.
This gives rise to multiple ways in which one can infer a new triple involving a given relation.
For example, we can use various properties of the relation \emph{isFatherOf} to do inference on (George H. W. Bush, \emph{isFatherOf}, ?).
If the knowledge graph contains another triple (George W. Bush, \emph{isChildrenOf}, George H. W. Bush), then we can utilize the information that the relation \emph{isChildrenOf} is the inverse relation of \emph{isFatherOf} to infer the missing entity.
If the above triple is missing, we could still utilize other interactions like (\emph{hasWife}, \emph{hasChildren}) $\Rightarrow$ \emph{isFatherOf} to infer the missing entity. 
Here, the context and interactions of entities and relations affect the logic we choose to infer a new triple. 

In this way, rather than a simple one-way interaction, there are various crossover interactions between entities and relations that affect the triples and inference of new links in knowledge bases.
In our opinion, using one general embedding for all interactions between entities and relations cannot model these crossover interactions.
To address this, our proposed model CrossE uses \emph{crossover interaction operation} to learn additional \emph{crossover interaction embeddings} of entities and relations. We describe them in detail in Section~\ref{sec:model}.
\end{comment}
%\CHJ{This section feels too weak.}




\begin{comment}

\section{Diversity of Semantic Representation}
Knowledge graph representation learning can achieve implicit reasoning during knowledge graph completion. Different semantics of relations support logic reasoning a lot and knowledge graph reprentation learning also should encode and discover latent semantics of relations existing in data.
If one semantic exist in both data and could be mapped to a specific axiom in ontology language then this semantic is important.
In this section we analyze the most common and important semantics for relations from the perspective of data, using FB15k as example, and ontology language using OWL 2 as example. 
\input{T-diverse-semantic}
%The OWL 2 Web Ontology Language, informally OWL 2, is an ontology language for the Semantic Web with formally defined meaning. We use some syntax from of OWL 2 as examples to illustrate the diversity of semantic in knolwedge base.
%We focus on two things during the analysis: 1) what is the requirement for score function designing to encode these semantic? 2) how to discovery the latent semantic?
%Each knowledge base embedding method has a score function $f()$ for every triplet to represent how likely the triplet is true. 

%definition / example / benefit for inference / OWL 2 axiom
Domain and range of a relation specify the class of head entity and tail entity should belong to and the correspond axiom in OWL 2 are \texttt{ObjectPropertyDomain()} and \texttt{ObjectPropertyRange()} respectively. Domain and range help filter irelevant entities and extract related information of head entity for a relation during the inference of a triple and most relations have latent domain and range.

The embedding of relations in knowledge graph representation learning method should be capable of catching the latent domain and range of the relations. The domain and range can be leverage to the entities to fectch relevant information of current triple. For example, if we want to know (Steven Spielberg, \emph{directedFilm}, ?), we first will search the related information of Steven Spielberg as a director rather information about his family, because the domain of \emph{directedFilm} is \emph{Director}. This illustrate that the relation will affect the information we search for entities during inference. So a representation learning method should have a gengeral embedding for enetities and multiple triple specific embeddings. 

Specific properties of relation help infer new triples if the properties are known. It is possible to combine implicit reasoning and logic reasoning together if a representation learning method can discover the properties of relations. 
Inverse relation specify the inverse relationship between two relations and the correspond axiom in OWL 2 is \texttt{InverseObjectProperty()}. For example, \emph{fatherOf} is the inverse relation of \emph{childrenOf}. Reflexive and symmetric relation specify that a relation is reflexive or symmetric and the corresponding axiom in OWL 2 is \texttt{RefxiveObjectProperty()} and \texttt{SymmetricObjectProperty} respectively. For example, relation \emph{knows} is a relfexive and \emph{hasSpouse} is symmetric. 
These properties are related with circle structures in graph and as proposed in \cite{}, to encode circle structures, a representation learning method should have different embeddings for an entity when as a head entity and as a tail entity with the same relation.
To discovery these properties, it is important to have an inverse embeddings for each relation which could be learned from head entity prediction. The similarity comparion between the embeding for relation and inverse relations can reveal the properties of relations. 

Caidinality constrains the number of tail entities for a relation. In OWL 2 there are three axiom related with cardinality as listed in \ref{diverse semantic}. According to the cardinality, all relations in knowledge graph could be classified into one of the four types: 1-1, 1-N, N-1 and N-N. Based on the diversity of cardinality, we regard the score function of triples as a soft constrain. \wen{need more explanation} But a basic assumption is that entity embeddings should be close to each other if they are similar in reality. 

In Table~\ref{diverse semantic}, we list the semantics talked in this section with data summary and their correspond OWL 2 axiom and condition to illustrate how these semantics support reasoning.  \texttt{CE} denotes a class expression. \texttt{OP} denotes an object property which is a relation called in this paper. \texttt{OPE} denotes an objective property experssion. $\centerdot ^\texttt{I}$ is the individual interpretation function and an individual is  an entity called in this paper. $\centerdot ^\texttt{C}$ and $\centerdot ^\texttt{OP}$ are class interpretation function and object property interpretation function respectively.


\CHJ{Could we add columns to Table 1 to list the capacity of existing models that can or can not deal with these types of semantics?}
%\subsection{Diversity of Entity Representation}

\CHJ{There are no definitions or description for terms such as OPE, CE in the table.}

\CHJ{Formal definitions for the semantics are better than plain descriptions.}

\end{comment}
%A class,  denoted with italic characters with the first character in upper case, is a set of entities with some properties in common.
%For example, if \emph{Doctor} is a class then each entity belong to this class should be a doctor.
%An entity could belong to more than one class. In the dataset about the class of entities in FB15k provided in \cite{TKRL:conf/ijcai/XieLS16}, each entity has $xx\%$ classes in average. For example, entity \emph{/m/064jjy}, which represents \emph{Peter Berg}, belongs to class \emph{/tv/tv\_director}, \emph{/film/actor} and \emph{/poeple/person} at the same time. 
%And different classes are about different aspects of an entity. Class \emph{/tv/tv\_director} and \emph{/film/actor} are related\wen{about?} with profession and \emph{/film/actor} is related with  more general information of a person, such as nationality or language. 
%In OWL 2, axiom \texttt{ClassAssertion()} is defined to specify the class of an entity.
%The class semantic\wen{?} gathers the entities with properties in common together and the domain/range of relations are also defined according to the class of subject and object. 

%\subsection{Domain/Range}
%Domain and range specify the class of subject and object for a relation should belong to.\wen{domain/range should be one class?} 
%For example, the domain of \emph{nationality} is \emph{Person} and the range is \emph{Country}. 
%In FB15k, $xx\%$ relations have explicit domain and range as the string of these relations are composed with three parts, the first part is related with domain, the second part is related with the predicate, and the third part is related with range.
%In OWL2, axiom \texttt{ObjectPropertyDomain()} and \texttt{ObjectPropertyRange()} are defined to specify the domain or range of a relation respectively. Dmoain and range  helps human filter irrelevant entities during triplet inference and the embedding model should encode this semantic.

%\subsection{Diversity of Relation Representation}

%\subsection{Domain/Range}
%Domain and range specify the class of subject and object for a relation should belong to.\wen{domain/range should be one class?} 
%For example, the domain of \emph{nationality} is \emph{Person} and the range is \emph{Country}. 
%In FB15k, $xx\%$ relations have explicit domain and range as the string of these relations are composed with three parts, the first part is related with domain, the second part is related with the predicate, and the third part is related with range.
%In OWL2, axiom \texttt{ObjectPropertyDomain()} and \texttt{ObjectPropertyRange()} are defined to specify the domain or range of a relation respectively. Dmoain and range  helps human filter irrelevant entities during triplet inference and the embedding model should encode this semantic.

%\subsection{Inverse relation}
%Inverse relation specify the inverse relationship between two relations. 
%For example, \emph{fatherOf} is the inverse relation of \emph{childrenOf}. 
%In theory, every relation has a inverse relation but not all inverse relations make sense. 
%In OWL 2, axiom \texttt{InverseObjectProperties()} is defined to specify the inverse relation for one relation.
%A lot triplet could be infered according to the inverse relationship of relations. 

%\subsection{Properties of relation}
%As proposed in \cite{ORC:conf/www/Zhang17}, there are three kind of properties of relations correspond to 'one-relation-circle' structures in knowledge base. Reflexive property is related to C1 structures, a circle strucutur including one kind entity and one kind relation. Symmetric property is related to C2 structures, a circle structure including two kind entities and one kind relation. Transitive properties is related to C3 structure including threee kind entities and one kind relation. There are $xx\%$, $xx\%$ and $xx\%$ relations are related to C1, C2 and C3 strutures in FB15k. In OWl 2, \texttt{RelfexiveObjectProperty()}, \texttt{SymmetricObjectProperty()} and \texttt{TransitiveObjectProperty()} are defined to specify the three kind properties of relations.
%The properties are important for relations and the embedding model should be capable to support correspond 'one-relation-circle' in order to encode the relations better and also should be capable to discover some properties of the relation.

%\subsection{Cardinality}
%Cardinality constrains the number of object for a relation. 
%In OWL2, there are three axioms related with cardinality, including \texttt{ObjectMinCardinality()}, \texttt{ObjectMaxCardinality} and \texttt{ObjectExactCardinality()} for the minmum object number, maximum object number and exact object number. According to the cardinality, the relations in knowledge base could be classified into four types: 1-1, 1-N, N-1 and N-N. The left number represent the average subject number per object and the right number represent the average object number per subject for one relation. 
%s cardinality is a basic perspective for relations, the embedding model should be capable to support all four types. 




